Structure and enumeration of (3+1)-free posets (extended abstract)

A poset is (3+1)-free if it does not contain the disjoint union of chains of length 3 and 1 as an induced subposet. These posets are the subject of the (3+1)-free conjecture of Stanley and Stembridge. Recently, Lewis and Zhang have enumerated \emph{graded} (3+1)-free posets, but until now the general enumeration problem has remained open. We enumerate all (3+1)-free posets by giving a decomposition into bipartite graphs, and obtain generating functions for (3+1)-free posets with labelled or unlabelled vertices.

==> header.tex <==
\pagestart{1}

\pageend{12}
\authorhead{Mathieu Guay-Paquet and Alejandro H. Morales and Eric Rowland}
\titlehead{Structure and enumeration of $(3+1)$-free posets (extended abstract)}
\titlelong{Structure and enumeration of $(3+1)$-free posets (extended abstract)}
\keywords{(3+1)-free posets, trace monoid, generating functions, chromatic symmetric function}


